Improving Hospital Mortality Prediction with Medical Named Entities and Multimodal Learning

Clinical text provides essential information to estimate the acuity of a patient during hospital stays in addition to structured clinical data. In this study, we explore how clinical text can complement a clinical predictive learning task. We leverage an internal medical natural language processing service to perform named entity extraction and negation detection on clinical notes and compose selected entities into a new text corpus to train document representations. We then propose a multimodal neural network to jointly train time series signals and unstructured clinical text representations to predict the in-hospital mortality risk for ICU patients. Our model outperforms the benchmark by 2% AUC.

==> conc.tex <==
Our work focuses on how to take advantage of free text, not just to prove the potential of clinical notes, but also explored how to use them effectively.
We show one way that utilizing text information to significantly boost in-hospital mortality prediction performance. Not only feeding the relevant information to train a note embedding, but also how to incorporate heterogeneous data into the network contributes to get a better performance. Our results are meaningful in a sense that we adopted the same data processing flow as the benchmark study to make fair comparison. 
On the other side, more accurate prediction on mortality in ICU can benefit nurses and physicians to have a better control of the acuity and potential outcomes of patients in early stage of admission.
In the future, we’d like to revisit incorporating notes information in the LSTM network with different model design. 

==> discussion.tex <==
We focus on how to use free text information to build competitive risk models. %not just to prove the potential of clinical notes, but also explored how to use them effectively.
Our results suggest the proposed multimodal neural network is more efficient to incorporate text information with structured data comparing to LSTM. Meanwhile, models using embeddings trained from medical named entities show consistent better performance than those trained from the simple tokenized text. Our results are straight comparable and reproducible by adopting the same data processing flow as the benchmark study. 
%On the other side, more accurate prediction on mortality in ICU can benefit healthcare providers to have a better control of the acuity and potential outcomes of patients in early stage of admission.
In the future, we’d like to further apply entity linking techniques to normalize extracted entities, and explore different models to incorporating notes information in the model, such as Bag of Words and CNN to study how to use clinical notes to enhance predictive modeling of clinical events. 

==> learning_old.tex <==
\subsection{Document Representation}

We used a skip-gram based document representation algorithm, Document Vector through Corruption (Doc2VecC) by \citet{cite-doc2vecc} to learn documents' embeddings. Doc2VecC algorithm represents each document by averaging over its word embeddings to reflect semantic meanings.

%\begin{figure}[h]
%\includegraphics[scale=.40]{doc2vec.png}
%\caption{Framework for learning document vectors.}
%\label{fig:doc2vec}
%\end{figure}
Different from previous work, corruption is added to the original document by randomly removing significant portion of words, and the document is represented using only the embeddings of the words remained. This corruption mechanism offers us great speedup during training as it significantly reduces the number of parameters to update in back propagation.
Another advantage of this method is that it is helpful to weigh down frequent words across document corpus, which brings great performance improvement. 



\subsection{Name Entity Recognition}
In this project, we constructed semantic notes using name entities extracted from original free text of clinical notes to train document embeddings as well. The motivation behind this approach is often times notes are full of noisy and redundant information. We want to see if training document embeddings on the top of text body composed of medical entities would reserve medical relevant information while achieving better performance.

The AWS medical NER system (\citet{amazonNER}) we used can be decomposed into three components: 1) the character-level encoder, which extracts features for each word from
characters, 2) the word-level encoder which extracts features from the surrounding sequence of words,
and 3) the tag decoder, which induces a probability distribution over any sequences of tags. \\ \\
\textbf{Character-Level Encoder} For each word i, we use CNNs, to extract character level
features 
(Figure 3). We apply ReLU nonlinearities  and dropout  between
CNN layers, and include a residual connection between input and output of each layer . So that our representation of the word is of fixed length, we apply max-pooling on the outputs
of the topmost layer of the character-level encoder. 
\begin{figure}[h]
\centering
\includegraphics[scale=.80]{char.png}
\caption{Example CNN architecture for Character-level Encoder with two layers.}
\label{fig:char}

\end{figure}

\textbf{Word-Level Encoder} To complete our representation of each word, we concatenate its character level
features with word embedding. 
We initialize the latent word embeddings with with word2vec training Mikolov et al. (2013) and then
update the embeddings over the course of training. In order to generalize to words unseen in the
training data, we replace each word with a special [UNK] (unknown) token with $50\%$ probability
during training. 
Given the sequence of word-level input features , we extract word-level hidden representations
for each word position in the sentence using a LSTM.
\begin{figure}[h]
\centering
\includegraphics[scale=.80]{wordlstm.png}
\caption{LSTM architecture for Word-level Encoder.}
\label{fig:word}

\end{figure}

\textbf{Tag Decoder} 
 The tag decoder induces a probability distribution over sequences of tags, conditioned
on the word-level encoder feature. we use an LSTM RNN for the tag decoder, as depicted in Figure 5. At the first time
step, the [GO]-symbol is provided as $y_1$ to the decoder LSTM. At each time step i, the LSTM
decoder computes $h^{Dec}_i+1$, the hidden state for decoding word ${i + 1}$, using the last tag $y_i$
, the current
decoder hidden state $h^{Dec}_i$
, and the learned representation of next word $h^{Enc}_{i+1}$. Using a softmax loss
function, $y_{i+1}$ is decoded; this is further fed as an input to the next time step.
\begin{figure}[h]
\centering
\includegraphics[scale=.80]{decode.png}
\caption{LSTM architecture for Tag Decoder.}
\label{fig:tag}
\end{figure}

\subsection{RNN with LSTM unit}
%Recurrent Neural Network (RNN) is a type of deep learning 
LSTM is one type of RNN and famously known for its capabilities to capture both long-term and short-term dependencies in sequence data (\citet{cite-lstm}). We used a LSTM variant with peephole connections (\citet{peepholeLSTM}).
Given a series of evenly spaced signals within a fixed observation window, $x=\{x_1, x_2, ..., x_T\}$, where $x_t \in \mathbf{R}^L$ and $L$ is the number of input signals, a hidden state vector $h_t$ can be learned at each time step $t$.

\begin{align*}
    h_1, ..., h_T &= LSTM(x_1, ..., x_T)
\end{align*}
%\begin{align*}
%    f_t &= \sigma(W_f\cdot[C_{t-1}, h_{t-1}, x_t] + b_f)\\
%    i_t &= \sigma(W_i\cdot[C_{t-1}, h_{t_1}, x_t] + b_i)\\
%    \Tilde{C}_t &= tanh(W_C\cdot[h_{t-1}, x_t] + b_C) \\
%    C_t &= f_t * C_{t-1} + i_t * \Tilde{C}_t \\
%    o_t &= \sigma(W_o[C_{t-1}, h_t-1, x_t] + b_o) \\
%    h_t &= o_t * tanh(C_t)
%\end{align*}


\subsection{Multimodal Learning}
%In order to compare performance cross different feature set, algorithms and model structures, it is important to compare models and methods on same data sets to arrive at a right conclusion. For this reason, we adopted the same data processing steps as \citet{cite-benchmark} for all the experiments carried on in this paper. Han
Multimodal deep learning frameworks was brought up by \citet{cite-multimodal}. When multiple modalities are available, fused representation can be used as input for discriminative tasks (\citet{multimodal-DBM}). 
We concatenated two days' embeddings $e_1$ and $e_2$, and passed it through one layer feedforward network to learn a hidden representation $h_e$. Further, a joint representation $h_j$ of clinical variables and text embeddings were learned from one layer feedforward network with concatenated vectors of last output from LSTM $h_T$ and $h_e$. Lastly, the representation passed though the output layer to predict class label $y \in {0, 1}$ indicating whether the patient encounter death before discharge.

\begin{align*}
    h_e &= W_e\cdot[e_1, e_2] + b_e\\
    h_j &= W_j\cdot[h_T, h_e] + b_j\\
    \hat{y} &= \sigma(W_y \cdot h_j + b_y)
\end{align*}

%The loss function :
%\begin{align*}
%    CE(y,\tilde{y}) = -(y \cdot log(\tilde{y})+(1-y) \cdot log(1-\tilde{y}))
%\end{align*}
%Include the diagram of the model architecture.

==> related.tex <==
Modern deep neural networks have been used to analyze a variety of human health data. In this section, we limit ourselves to review of data generated by hospitals.
\paragraph{Deep Neural Networks in Healthcare.}
Recurrent Neural Networks (RNN) and their variants such as Long Short-Term Memory (LSTM) were some of the earliest deep neural networks to be used for analysis of patient vital signs and signals recorded in the hospital \citep{LiptonKEW15,che2016recurrent}. They were also used to analyze higher dimensional structured claims data \citep{choi2016doctor}. In both cases, the learning objective was either to stratify patients based on their risks or predict the diagnosis or prognosis. Medical notes are believed to be a rich source of patient health information and analyzed commonly via RNNs to extract insights \citep{rumshisky2016predicting,CaballeroBarajas2015,Ghassemi2015AMT,Suresh2017ClinicalIP}. Convolutional architechtures also have been found to be faster and achieve similar accuracy \citep{razavian2016multi}. For the full list of contributions in this field, we refer to the recent survey papers \citep{miotto2017deep}. \textbf{[Taha]: More papers will be added}
% lipton2015learning, choi2016doctor, razavian2016multi, che2016recurrent, miotto2017deep, suresh2017clinical, rajkomar2018scalable
\paragraph{Multi-modal Analysis.} 
Using multiple data modes to assess the patients risk can potentially improve the 
In order to compare performance cross different feature set, algorithms and model structures, it is important to compare models and methods on same data sets to arrive at a right conclusion. For this reason, we adopted the same data processing steps as \citet{cite-benchmark} for all the experiments carried on in this paper. Han

Cite a couple of papers. Refer to Google's paper for the challenges.

\citep{ghassemi2014unfolding}: Topic modeling, concatenation, non-temporal (look at the references of this paper and cite them)

\citep{ghassemi2015multivariate}: Topic modeling, MTGP, temporal


